Circular Quasiconformal Deturbulence: Geometry-Based Restoration from Multiple Turbulent Frames

Imaging through inhomogeneous media often results in severe distortions, posing significant challenges to downstream image-processing tasks. The lack of clean paired images makes supervised learning impractical, motivating unsupervised restoration approaches. In this work, we propose the Circular Quasi-Conformal Deturbulence (CQCD) framework, an unsupervised approach that reconstructs distortion-free images from multiple frames using a circular architecture. The framework minimizes reconstruction errors by jointly estimating forward and backward transformations between distorted observations and the restored image. A key advancement of CQCD is the integration of computational quasi-conformal geometry, which encourages bijective non-rigid deformations and improves the well-posedness of both forward and inverse mappings for cycle consistency. The deformation field is further regularized to preserve structural coherence and reduce non-physical artifacts such as folding or tearing. Additionally, tight-frame blocks are employed to effectively encode distortion-sensitive features, enhancing the precision of the restoration process. To assess the effectiveness of the proposed framework, extensive evaluations are conducted on synthetic and real-world image datasets. Experimental findings indicate that CQCD not only surpasses existing state-of-the-art deturbulence techniques in restoration quality but also achieves highly accurate deformation field estimation.

==> theorem.tex <==
Let $D$ be the bounded component of $\mathbb C\setminus \Gamma$. Since $\mu=f_{\bar z}/f_z$ is well defined, we have $f_z\neq 0$ in $\Omega$. Moreover,
$$J_f=|f_z|^2-|f_{\bar z}|^2
=|f_z|^2(1-|\mu|^2)>0,$$
because $\|\mu\|_\infty<1$. Hence $Df$ is nonsingular everywhere in $\Omega$, and by the inverse function theorem,
$$f|_\Omega:\Omega\to \mathbb C$$
is a local $C^1$-diffeomorphism, in particular a local homeomorphism.
By the standard degree formula for planar maps, $f|_{\partial\Omega}$ determines degree $1$ on $D$ and degree $0$ on the exterior of $\Gamma$; since $J_f>0$, all local degrees are positive, so no exterior point has a preimage. Therefore
$$f(\Omega)\subset D.$$
Thus we may regard
$$g:=f|_\Omega:\Omega\to D.$$
We now apply Ho’s global inversion criterion: a proper local homeomorphism whose induced map on fundamental groups is surjective is a global homeomorphism. The map $g$ is proper. Indeed, if $K\subset D$ is compact, then $f^{-1}(K)$ is closed in $\overline{\Omega}$, hence compact. Moreover,
$$f^{-1}(K)\cap \partial\Omega=\varnothing,$$
because $f(\partial\Omega)=\Gamma$ and $K\cap\Gamma=\varnothing$. Hence $g^{-1}(K)$ is compact in $\Omega$.
Since $\Omega$ is a Jordan domain and $D$ is the bounded component enclosed by the Jordan curve $\Gamma$, both $\Omega$ and $D$ are homeomorphic to the unit disk. Therefore
$$\pi_1(\Omega)=0,
\qquad
\pi_1(D)=0,$$
so the induced homomorphism
$$g_*:\pi_1(\Omega)\to\pi_1(D)$$
is automatically surjective. Ho’s theorem then implies that
$$g=f|_\Omega:\Omega\to D$$
is a homeomorphism.
Finally, $f|_{\partial\Omega}:\partial\Omega\to\Gamma$ is a homeomorphism by assumption, while
$$f(\Omega)=D,\qquad f(\partial\Omega)=\Gamma.$$
Hence
$$f:\overline{\Omega}\to\overline D$$
is a continuous bijection. Since $\overline{\Omega}$ is compact and $\overline D$ is Hausdorff, this continuous bijection is a homeomorphism. Therefore
$$\boxed{f:\overline{\Omega}\to\overline D\text{ is a homeomorphism}.}$$
Citation for the global inversion step:

% \begin{theorem}[Bijectivity on a bounded image domain]\label{thm:bounded-qc-bijective}
% Let $\Omega\subset\mathbb C$ be a bounded Jordan domain (in particular, a square domain is allowed), and
% let
% \[
% f\in C(\overline{\Omega})\cap C^{1}(\Omega).
% \]
% Assume:

% \begin{enumerate}
% \item $f_{z}(z)\neq 0$ for every $z\in\Omega$, and
% \[
% \mu(z):=\frac{f_{\bar z}(z)}{f_{z}(z)}
% \quad\text{satisfies}\quad
% \|\mu\|_{L^\infty(\Omega)}<1;
% \]
% \item the boundary map
% \[
% f|_{\partial\Omega}:\partial\Omega\to\Gamma
% \]
% is an orientation-preserving homeomorphism onto a Jordan curve $\Gamma$.
% \end{enumerate}

% Let $D:=\operatorname{int}\Gamma$ be the bounded component of $\mathbb C\setminus\Gamma$.
% Then
% \[
% f:\overline{\Omega}\to\overline{D}
% \]
% is a homeomorphism. In particular, $f$ is bijective from $\overline{\Omega}$ onto $\overline D$, and
% $f|_{\Omega}:\Omega\to D$ is bijective.
% \end{theorem}

% \begin{proof}
% Since $\mu=f_{\bar z}/f_z$ and $\|\mu\|_\infty<1$, for every $z\in\Omega$,
% \[
% J_f(z)=|f_z(z)|^2-|f_{\bar z}(z)|^2
%       =|f_z(z)|^2\bigl(1-|\mu(z)|^2\bigr)>0.
% \]
% Hence $Df(z)$ is invertible at each $z\in\Omega$, so by the inverse function theorem
% $f|_\Omega$ is a local $C^1$-diffeomorphism, in particular a local homeomorphism and an open map.

% Now compare Brouwer degrees using the boundary map.
% Because $f|_{\partial\Omega}$ is an orientation-preserving homeomorphism onto $\Gamma$, for $y\notin\Gamma$,
% \[
% \deg(f,\Omega,y)=
% \begin{cases}
% 1,& y\in D,\\
% 0,& y\in \mathbb C\setminus \overline D.
% \end{cases}
% \]
% Fix $y\in \mathbb C\setminus \overline D$. If $y=f(x)$ for some $x\in\Omega$, then each preimage contributes
% positive local degree (since $J_f>0$), so $\deg(f,\Omega,y)>0$, contradicting $\deg(f,\Omega,y)=0$.
% Therefore
% \[
% f(\Omega)\subset D.
% \]
% Define
% \[
% g:=f|_\Omega:\Omega\to D.
% \]

% We claim that $g$ is proper.
% Let $K\subset D$ be compact.
% Then $g^{-1}(K)=f^{-1}(K)\cap\Omega$.
% Since $f$ is continuous on $\overline\Omega$, $f^{-1}(K)$ is closed in $\overline\Omega$; thus it is compact
% (because $\overline\Omega$ is compact).
% Also
% \[
% f^{-1}(K)\cap\partial\Omega=\varnothing,
% \]
% because $f(\partial\Omega)=\Gamma$ and $K\cap\Gamma=\varnothing$.
% Hence $g^{-1}(K)=f^{-1}(K)$ is compact in $\Omega$.
% So $g$ is proper.

% Therefore $g$ is a proper local homeomorphism.
% A proper local homeomorphism into a Hausdorff space is closed, and a local homeomorphism is open; hence
% $g(\Omega)$ is both open and closed in the connected set $D$.
% Since $g(\Omega)\neq\varnothing$, we get $g(\Omega)=D$, i.e. $g$ is surjective.

% Now $g:\Omega\to D$ is a surjective proper local homeomorphism, hence a covering map.
% Because $D$ is a Jordan domain, it is simply connected; thus any connected covering over $D$ has one sheet.
% So $g$ is a homeomorphism $\Omega\to D$.

% Finally, we already have:
% \[
% f|_{\Omega}:\Omega\to D \text{ is a homeomorphism},\qquad
% f|_{\partial\Omega}:\partial\Omega\to\Gamma \text{ is a homeomorphism},
% \]
% and $D\cap\Gamma=\varnothing$.
% Hence $f:\overline\Omega\to\overline D$ is bijective.
% It is continuous by assumption, and $\overline\Omega$ is compact while $\overline D$ is Hausdorff, so
% a continuous bijection is a homeomorphism.
% Therefore
% \[
% f:\overline\Omega\to\overline D
% \]
% is a homeomorphism.
% \end{proof}
